Efficient solution strategies for cabin noise assessment of a wave resolving aircraft fuselage model

For the purpose of high-fidelity aircraft cabin noise simulations during early design phases, we study three efficient solving approaches for the fully coupled finite element model of an aircraft fuselage segment. Obtaining an efficient solution with respect to consumed computational time and resources is challenging within a conventional simulation pipeline, as large-scale and complex vibroacoustic models demand crucially high computational costs with increasing frequency. In this contribution, we adopt (1) frequency and domain-adaptive discretisation, (2) domain-decomposition techniques, and (3) model order reduction with rational Arnoldi Krylov subspace methods for an aircraft fuselage model. The three approaches have shown remarkable advantage thereby reducing the solving time as well as the memory requirement that are essential when solving large-scale models. While the discretisation and the model order reduction approaches accelerate the solving process by efficiently handling the complexity of the system to be solved, domain-decomposition techniques further handle the aspect of reducing the overall memory consumption. Finally with the help of active research aircraft models, we implement and showcase the achieved efficiency.

==> images/FEmatrices.tex <==
%\tikzsetnextfilename{aircraft_core_FEmodel}
\begin{tikzpicture}
\node[inner sep=0pt, align=left] (bild) at (0,0)  {\includegraphics[width=\textwidth]{./images/FEmatrices.png}};  
\node[fill=white,draw=black,rounded corners=3pt,inner sep=3pt, align=left, anchor=center] (lab1) at (-0.3\textwidth,0.15\textwidth) {$\Omega_\mathrm{1}$}; 
\node[fill=white,draw=black,rounded corners=3pt,inner sep=3pt, align=left, anchor=center] (lab2) at (-0.23\textwidth,0.01\textwidth) {$\Omega_\mathrm{2}$}; 
\node[fill=white,draw=black,rounded corners=3pt,inner sep=3pt, align=left, anchor=center] (lab2) at (-0.15\textwidth,-0.06\textwidth) {$\Omega_\mathrm{3}$}; 
\node[fill=white,draw=black,rounded corners=3pt,inner sep=3pt, align=left, anchor=center] (lab2) at (-0.15\textwidth,-0.15\textwidth) {$\Omega_\mathrm{4}$}; 
%
\end{tikzpicture}

==> images/FEmatrices2.tex <==
%\tikzsetnextfilename{aircraft_core_FEmodel}
\begin{tikzpicture}
\node[inner sep=0pt, align=left] (bild) at (0,0)  {\includegraphics[width=0.35\textwidth]{./images/FEmatrices2.png}};  
%
\end{tikzpicture}

==> images/pyplots/mor_convergence/plt_errorconv_size_258.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color3}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}
\definecolor{color4}{rgb}{0.505882352941176,0.447058823529412,0.701960784313725}
\definecolor{color5}{rgb}{0.576470588235294,0.470588235294118,0.376470588235294}
\definecolor{color6}{rgb}{0.854901960784314,0.545098039215686,0.764705882352941}

\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xlabel=\textcolor{white!15!black}{ROM dimension},
xmajorgrids,
xmin=126, xmax=654,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel=\textcolor{white!15!black}{Maximum relative error},
ymajorgrids,
ymin=0.00191477117555678, ymax=2.24301350199255,
ymode=log,
ytick style={color=white!15!black}
]
\addplot [very thick, color0, mark=square*, mark size=3, mark options={solid,draw=white}]
table {%
260 1.62684
470 0.0386172
490 0.00551
};
\addlegendentry{fROM-1}
\addplot [very thick, color1, mark=square*, mark size=3, mark options={solid,draw=white}]
table {%
170 0.299177
330 0.277737
500 0.0376289
620 0.039969
630 0.00821
};
\addlegendentry{fROM-2}
\addplot [very thick, color2, mark=square*, mark size=3, mark options={solid,draw=white}]
table {%
170 0.19773
330 0.703398
500 0.0547428
610 0.00503
};
\addlegendentry{fROM-3}
\addplot [very thick, color3, mark=square*, mark size=3, mark options={solid,draw=white}]
table {%
150 0.0788685
290 0.823862
440 0.0151848
570 0.0058142
};
\addlegendentry{fROM-4}
\addplot [very thick, color4, mark=square*, mark size=3, mark options={solid,draw=white}]
table {%
150 0.0713064
290 0.0722103
430 0.0419048
530 0.0750658
540 0.00264
};
\addlegendentry{fROM-5}
\addplot [very thick, color5, mark=square*, mark size=3, mark options={solid,draw=white}]
table {%
160 0.0568613
300 0.053031
450 0.0159498
550 0.006591
};
\addlegendentry{fROM-6}
\addplot [very thick, color6]
table {%
150 0.01
630 0.01
};
\addlegendentry{Tolerance}
\end{axis}

\end{tikzpicture}


==> images/pyplots/mor_eigs/plt_eigdensity.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}

\begin{axis}[
axis line style={white!15!black},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xlabel=\textcolor{white!15!black}{Frequency (Hz)},
xmajorgrids,
xmin=-39.5, xmax=1049.5,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel=\textcolor{white!15!black}{Modal density},
ymajorgrids,
ymin=0, ymax=4100,
ytick style={color=white!15!black}
]
\addplot [very thick, color0]
table {%
10 0
12 0
14 0
16 0
18 0
20 0
22 0
24 0
26 0
28 0
30 0
32 0
34 0
36 0
38 0
40 0
42 0
44 0
46 0
48 0
50 0
52 0
54 0
56 0
58 0
60 0
62 0
64 0
66 0
68 0
70 0
72 0
74 0
76 0
78 0
80 0
82 0
84 0
86 0
88 0
90 0
92 0
94 0
96 0
98 0
100 0
102 0
104 0
106 0
108 0
110 0
112 0
114 0
116 0
118 0
120 0
122 0
124 0
126 0
128 0
130 0
132 0
134 0
136 0
138 0
140 0
142 0
144 0
146 0
148 0
150 0
152 0
154 0
156 0
158 0
160 0
162 0
164 0
166 0
168 0
170 0
172 0
174 0
176 0
178 0
180 0
182 0
184 0
186 0
188 0
190 0
192 0
194 0
196 0
198 0
200 0
202 0
204 0
206 0
208 0
210 0
212 0
214 0
216 0
218 0
220 0
222 0
224 0
226 0
228 0
230 0
232 0
234 0
236 0
238 0
240 0
242 0
244 0
246 0
248 0
250 0
252 0
254 0
256 0
258 0
260 0
262 0
264 0
266 0
268 0
270 0
272 0
274 0
276 0
278 0
280 0
282 0
284 0
286 0
288 0
290 0
292 0
294 0
296 0
298 0
300 0
302 0
304 0
306 0
308 0
310 0
312 0
314 0
316 0
318 0
320 0
322 0
324 0
326 0
328 0
330 0
332 0
334 0
336 0
338 0
340 0
342 0
344 0
346 0
348 0
350 0
352 0
354 0
356 0
358 0
360 0
362 0
364 0
366 0
368 0
370 0
372 0
374 0
376 0
378 0
380 0
382 0
384 0
386 0
388 0
390 0
392 0
394 0
396 0
398 0
400 0
402 0
404 0
406 0
408 0
410 0
412 0
414 0
416 0
418 0
420 0
422 0
424 0
426 0
428 0
430 0
432 0
434 0
436 0
438 0
440 0
442 0
444 0
446 0
448 0
450 0
452 0
454 0
456 0
458 0
460 0
462 0
464 0
466 0
468 0
470 0
472 0
474 0
476 0
478 0
480 0
482 0
484 0
486 0
488 0
490 0
492 0
494 0
496 0
498 0
500 0
502 0
504 0
506 0
508 0
510 0
512 0
514 0
516 0
518 0
520 0
522 0
524 0
526 0
528 0
530 0
532 0
534 0
536 0
538 0
540 0
542 0
544 0
546 0
548 0
550 0
552 0
554 0
556 0
558 0
560 0
562 0
564 0
566 0
568 0
570 0
572 0
574 0
576 0
578 0
580 0
582 0
584 0
586 0
588 0
590 0
592 0
594 0
596 0
598 0
600 0
602 0
604 0
606 0
608 0
610 0
612 0
614 0
616 0
618 0
620 0
622 0
624 0
626 0
628 0
630 0
632 0
634 0
636 0
638 0
640 0
642 0
644 0
646 0
648 0
650 0
652 0
654 0
656 0
658 0
660 0
662 0
664 0
666 0
668 0
670 0
672 0
674 0
676 0
678 0
680 0
682 0
684 0
686 0
688 0
690 0
692 0
694 0
696 0
698 0
700 0
702 0
704 0
706 0
708 0
710 0
712 0
714 0
716 0
718 0
720 0
722 0
724 0
726 0
728 0
730 0
732 0
734 0
736 0
738 0
740 0
742 0
744 0
746 0
748 0
750 0
752 0
754 0
756 0
758 0
760 0
762 0
764 0
766 0
768 0
770 0
772 0
774 0
776 0
778 0
780 0
782 0
784 0
786 0
788 0
790 0
792 0
794 0
796 0
798 0
800 0
802 0
804 0
806 0
808 0
810 0
812 0
814 0
816 0
818 0
820 0
822 0
824 0
826 0
828 0
830 0
832 0
834 0
836 0
838 0
840 0
842 0
844 0
846 0
848 0
850 0
852 0
854 0
856 0
858 0
860 0
862 0
864 0
866 0
868 0
870 0
872 0
874 0
876 0
878 0
880 0
882 0
884 0
886 0
888 0
890 0
892 0
894 0
896 0
898 0
900 0
902 0
904 0
906 0
908 0
910 0
912 0
914 0
916 0
918 0
920 0
922 0
924 0
926 0
928 0
930 0
932 0
934 0
936 0
938 0
940 0
942 0
944 0
946 0
948 0
950 0
952 0
954 0
956 0
958 0
960 0
962 0
964 0
966 0
968 0
970 0
972 0
974 0
976 0
978 0
980 0
982 0
984 0
986 0
988 0
990 0
992 0
994 0
996 0
998 0
1000 0
};
\end{axis}

\end{tikzpicture}


==> images/pyplots/mor_tfs/plt_transferfunction_AIR_258.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}

\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis y={10},
tick align=outside,
tick pos=left,
title={FRF},
x grid style={white!80!black},
xlabel=\textcolor{white!15!black}{Frequency (Hz)},
xmajorgrids,
xmin=-2.4, xmax=270.4,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel=\textcolor{white!15!black}{Transfer function},
ymajorgrids,
ymin=0.0035551763202869, ymax=0.905860114396819,
ymode=log,
ytick style={color=white!15!black}
]
\addplot [thick, color0]
table {%
10 0.00635854089907965
12 0.00598960583982924
14 0.00596076075769606
16 0.0074116500487623
18 0.00586980179894291
20 0.00457420361841788
22 0.00510741725333997
24 0.0104269700035688
26 0.0284500807295291
28 0.0910079077389671
30 0.0687883371089669
32 0.049835900048695
34 0.0450909792171513
36 0.044782450012697
38 0.0449342574252432
40 0.0481782518739169
42 0.0554862976103876
44 0.0683897604810362
46 0.0928964733113226
48 0.14463594211633
50 0.268959762211227
52 0.704187659271309
54 0.241552509067974
56 0.137311857642768
58 0.10399236773566
60 0.0784947704990923
62 0.0323193618519239
64 0.0343235976447088
66 0.055404399435006
68 0.12734233563668
70 0.184968704266659
72 0.240108968160105
74 0.370425910136723
76 0.267745729879621
78 0.144526786604676
80 0.102650548902013
82 0.0895312919231831
84 0.0829521238020843
86 0.0755178125307041
88 0.0714195484335543
90 0.0671890517053636
92 0.0555412489235168
94 0.0880350695213396
96 0.0752967086655262
98 0.0910737687726545
100 0.121476502490517
102 0.101387764912088
104 0.0719654933830094
106 0.0469925380098012
108 0.0326432374617971
110 0.0280271185484576
112 0.0327111271430088
114 0.0447322079034419
116 0.0585189799981849
118 0.0572258779939284
120 0.0260955619963935
122 0.0190083556597396
124 0.0253452495472647
126 0.0311367992682759
128 0.0446025409299888
130 0.0662215087399173
132 0.107259961024028
134 0.202643679530875
136 0.457387824963425
138 0.509443307131334
140 0.413942712352917
142 0.41340640693873
144 0.292476959098898
146 0.15522143203484
148 0.0976934386714434
150 0.0767195434080074
152 0.0641813049448335
154 0.0497942372641951
156 0.0344479305100691
158 0.0717006576282825
160 0.10734418325149
162 0.117094489271875
164 0.106379247446133
166 0.073277033195739
168 0.0368308373419606
170 0.0347259317699161
172 0.0113263376725493
174 0.0153100980683777
176 0.0301885888045492
178 0.0249721051958473
180 0.017973248880182
182 0.0179029350530703
184 0.058322373908492
186 0.0675617907437456
188 0.0769764872496635
190 0.0735337036656544
192 0.0566721351766593
194 0.0426343291395654
196 0.0329864805882787
198 0.027779306096092
200 0.0267063165730406
202 0.0277821224721485
204 0.0326793164608403
206 0.0453176209054133
208 0.0674447925506408
210 0.0879831740583743
212 0.0800606548020509
214 0.0653248340111519
216 0.0569625976312271
218 0.0529204180353403
220 0.0530485806381931
222 0.0570517155658915
224 0.0659757928508151
226 0.0803074864339743
228 0.103406886967641
230 0.142226238631801
232 0.167671704000947
234 0.144724394657645
236 0.11925047632447
238 0.165882527666497
240 0.120505448934956
242 0.192040342823743
244 0.32887582987501
246 0.375591422587587
248 0.346755572434935
250 0.231659510820463
252 0.147866575484013
254 0.123941829092003
256 0.115415393319697
258 0.0816398478277853
};
\addlegendentry{FOM}
\addplot [thick, color1, dashed]
table {%
10 0.00635854074232169
12 0.00598986946912733
14 0.00596094144682445
16 0.00741003492399732
18 0.00586810277108934
20 0.00457334402083458
22 0.00510811292821422
24 0.0104279301186353
26 0.0284502141172066
28 0.0910079076292808
30 0.0687842748921675
32 0.0498335788738236
34 0.0450870978081721
36 0.0447797492164465
38 0.0449374348578137
40 0.0481714291938314
42 0.0554698004381658
44 0.0683639434093566
46 0.092879287120591
48 0.144660649447532
50 0.268959762287736
52 0.704187660828596
54 0.241547157123516
56 0.137424442059497
58 0.103937952514833
60 0.0785680047908746
62 0.0355415068424839
64 0.0339767243022898
66 0.0554044014162517
68 0.127518811045349
70 0.184915509564635
72 0.23998392127123
74 0.370425915235003
76 0.26765008206295
78 0.144424636833327
80 0.102477507664265
82 0.0890759877218421
84 0.0822316898335092
86 0.0752662813748105
88 0.0714645673705254
90 0.0670208969150754
92 0.0555412482238712
94 0.0869777624254946
96 0.0752342824840455
98 0.0911907291747317
100 0.121476502982665
102 0.101474948871188
104 0.0718064210817853
106 0.0468936420611834
108 0.0326070780235245
110 0.0280285121499046
112 0.0327086606302936
114 0.0446017770613865
116 0.0583822834924075
118 0.0572258773955079
120 0.0262851624027427
122 0.0190299729746447
124 0.0253909260470745
126 0.0310165211667977
128 0.0445107865664868
130 0.0661560801594907
132 0.107236368195822
134 0.202643680845837
136 0.457247731730798
138 0.5094433179624
140 0.41394271801293
142 0.41378728150791
144 0.292748348976024
146 0.154983355769357
148 0.097321445260259
150 0.0760901915482398
152 0.0641813020927544
154 0.0502855141692726
156 0.0355793177334548
158 0.0706616472691505
160 0.107344183727576
162 0.119402500788448
164 0.110410990020259
166 0.0764538913295208
168 0.0411198185068284
170 0.0347554601652351
172 0.0110619700179877
174 0.0169313721059951
176 0.030970283707658
178 0.0278332034384692
180 0.0224162341304243
182 0.01790293454517
184 0.0502363920958871
186 0.059961290387747
188 0.0707357736019613
190 0.0711583485286656
192 0.0568557451905207
194 0.0430284525197328
196 0.0337803166513417
198 0.0285737150138512
200 0.0274503211131853
202 0.0284604824500393
204 0.0335314563042617
206 0.0463297912999057
208 0.0681300087657041
210 0.0879831320367599
212 0.0797349427619491
214 0.0650281847689367
216 0.0565699084852267
218 0.0526762928793251
220 0.0529773176318584
222 0.0575398311868488
224 0.0670619229307091
226 0.081274401708041
228 0.103673505223413
230 0.142226236031801
232 0.167670475387985
234 0.144405381475672
236 0.118830426537083
238 0.165882526881076
240 0.120364525033291
242 0.192040342397745
244 0.328875827631559
246 0.375591423733487
248 0.346755573135168
250 0.231753929853017
252 0.147416858529089
254 0.122675901539651
256 0.114573644177855
258 0.0816401506815567
};
\addlegendentry{ROM}
\end{axis}

\end{tikzpicture}

